Dual Geometric Graph Network (DG2N) -- Iterative network for deformable shape alignment

We provide a novel new approach for aligning geometric models using a dual graph structure where local features are mapping probabilities. Alignment of non-rigid structures is one of the most challenging computer vision tasks due to the high number of unknowns needed to model the correspondence. We have seen a leap forward using DNN models in template alignment and functional maps, but those methods fail for inter-class alignment where nonisometric deformations exist. Here we propose to rethink this task and use unrolling concepts on a dual graph structure - one for a forward map and one for a backward map, where the features are pulled back matching probabilities from the target into the source. We report state of the art results on stretchable domains alignment in a rapid and stable solution for meshes and cloud of points.

==> Sections/Background/3d_shape_corr/feature_matching.tex <==
\paragraph{Feature matching}
One popular method of minimizing \ref{eq:min_dist_corr}without computing all $|\source|^{|\target|}$ matches is to consider only matches among points with similar descriptors; In doing so, the key problem now turns into creating descriptive deformation-invariant local point features instead of solving the non-linear objective function.
This has been a key research goal in shape analysis with a great impact on the community. Some examples include GPS \cite{gps}, SHOT\cite{shot} and spectral signatures \cite{hks,wks}. Rotation-invariant descriptors have also been suggested\cite{shot,rotinv}, As this is an important attribute for 3d shape analysis.
These handcrafted descriptors usually require a significant amount of manual tuning and do not work well when applied in different settings.
Lately, a tremendous amount of research has been devoted to \textbf{learning} point descriptors, with methods ranging from random forests \cite{randomforest} to metric learning \cite{meta}.
In more recent years, the field of deep-learning showed remarkable results for 3d point-descriptors as well \cite{pointnet,dgcnn,fmnet,3dcoded}, Providing state-of-the-art solutions for 3d registration.
As we will prove, local learnable descriptors are not sufficient as a holistic solution due to data-variations, noise, and sensitivity for complex deformations.

==> Sections/Background/3d_shape_corr/unsup_corr.tex <==
\paragraph{Unsupervised and zero-shot dense shape correspondence}
Solving machine learning problems in an unsupervised fashion is marked as one of our community's most significant future goals.
For the dense shape correspondence problem, only a limited set of methods proposed such unsupervised learning mechanisms, among them are \cite{3dcoded,halimi,dvir,surfmnet}.

The first work \cite{3dcoded} used a template that closely resembles all shapes in the dataset and tried to map each vertex of a shape to a vertex in the template using an auto-encoder; at inference, the pair correspondence is $\pi^{-1}_{\target}(\pi_{\source}(x_i))$
where $\pi_{\target}$ is the mapping from shape $\target$ to the template. This method requires a great amount of training data and fail on datasets where no "natural" template can be defined.
Other works such as Ginzburg \& Raviv \cite{dvir} optimize for a smooth cyclic mapper, where the objective of the bi-directional mapper is to map each vertex to itself after a full cyclic.

A groundbreaking subdomain in unsupervised learning is zero-shot learning, where a model can complete a task by only examining the test-sample itself \cite{zeroshot1,zeroshot2}.
One of the first methods to suggest such a framework for zero-shot alignment \cite{halimi} worked in the spectral domain and tried to minimize the distortion function on the inference pair directly using gradient descent on the point descriptors until convergence. Halimi \etal \cite{halimi} and works that followed \cite{dvir} only worked with nearly-isometric shapes, heavily influenced by the shapes' topology and data's modality. 

All mentioned works have opened the door to a new era of shape registration but still shows some gap from their supervised counterparts.
Here, we show how modeling the correspondence itself as an input to the learning pipeline allows the network to overcome problems that previous unsupervised methods encountered.


==> Sections/Background/refinment_illustration_fig.tex <==

\begin{figure*}[!th]
\centering % <-- added
  \begin{subfigure}{0.23\textwidth}
    \centering
  \includegraphics[width=3.5cm]{Sections/Experiments/images/self_sup/refinment_faust/human_reference.png}
%   \caption{Reference}
    \label{fig:refine0}
  \end{subfigure}\hfil
    \begin{subfigure}{0.23\textwidth}
    \centering
  \includegraphics[width=3.5cm]{Sections/Experiments/images/self_sup/refinment_faust/human0.png}
%   \caption{14.5 MGE}
    \label{fig:refine1}
  \end{subfigure}\hfil
%     \begin{subfigure}{0.23\textwidth}
%     \centering
%   \includegraphics[width=3.5cm]{Sections/Experiments/images/self_sup/refinment_faust/ep_0_src_7574_tgt_14771_new_new_cur_path_10.png}
% %   \caption{Step 2}
%     \label{fig:refine21}
%   \end{subfigure}\hfil
    \begin{subfigure}{0.23\textwidth}
    \centering
  \includegraphics[width=3.5cm]{Sections/Experiments/images/self_sup/refinment_faust/human3.png}
%   \caption{9.8 MGE}
    \label{fig:refine3}
  \end{subfigure}\hfil
%       \begin{subfigure}{0.23\textwidth}
%     \centering
%   \includegraphics[width=3.5cm]{Sections/Experiments/images/self_sup/refinment_faust/ep_0_src_7574_tgt_14771_new_new_cur_path_40.png}
% %   \caption{Step 4}
%     \label{fig:refine4}
%   \end{subfigure}\hfil
      \begin{subfigure}{0.23\textwidth}
    \centering
  \includegraphics[width=3.5cm]{Sections/Experiments/images/self_sup/refinment_faust/human5.png}
%   \caption{3.2 MGE}
    \label{fig:refine5}
  \end{subfigure}\hfil
  \medskip
  
    \begin{subfigure}{0.23\textwidth}
    \centering
  \includegraphics[width=4.1cm]{Sections/Experiments/images/self_sup/refinment_smal/horseref.PNG}
  \caption{Reference}
    \label{fig:refine00}
  \end{subfigure}\hfil
    \begin{subfigure}{0.23\textwidth}
    \centering
  \includegraphics[width=3.5cm]{Sections/Experiments/images/self_sup/refinment_smal/cat0.PNG}
  \caption{Step 1}
    \label{fig:refine11}
  \end{subfigure}\hfil
%     \begin{subfigure}{0.23\textwidth}
%     \centering
%   \includegraphics[width=3.5cm]{Sections/Experiments/images/self_sup/refinment_smal/02.PNG}
%   \caption{Step 2}
%     \label{fig:refine22}
%   \end{subfigure}\hfil
    \begin{subfigure}{0.23\textwidth}
    \centering
  \includegraphics[width=3.7cm]{Sections/Experiments/images/self_sup/refinment_smal/cat3.PNG}
  \caption{Step 3}
    \label{fig:refine33}
  \end{subfigure}\hfil
%       \begin{subfigure}{0.23\textwidth}
%     \centering
%   \includegraphics[width=3.5cm]{Sections/Experiments/images/self_sup/refinment_smal/04.PNG}
%   \caption{Step 4}
%     \label{fig:refine44}
%   \end{subfigure}\hfil
      \begin{subfigure}{0.23\textwidth}
    \centering
  \includegraphics[width=3.5cm]{Sections/Experiments/images/self_sup/refinment_smal/cat5.PNG}
  \caption{Step 5}
    \label{fig:refine55}
  \end{subfigure}\hfil
  \medskip
  
  \caption{Refinement illustration - self supervised setting. Given two input shapes we use SURFMNet as the initiator, and present here the refinement steps, leftmost - correspondence output from SURFMNet, rightmost - correspondence after 5 refinement steps of DG2N.\\ Mean geodesic error over time FAUST - SURFMNet 18.5, First iteration 13.7, Third iteration 8.8, Fifth iteration 3.7.\\
   Mean geodesic error over time SMAL - SURFMNet 14.3, First iteration 9.5, Third iteration 6.2, Fifth iteration 4.1.}
  \label{fig:refinment}
\end{figure*}


==> Sections/Method/graph_denosing.tex <==
\paragraph{Graph denoising}\label{subsec:denoise}
We assume $\softP$ and $\softP^T$ are noisy or approximate solutions to the dense shape correspondence and present a method of deriving the underlying mapping.
The maximum likelihood solution for the mapping from $\softP$ is  $$MLE(\pi(x_i))=\argmax_{j^*}(P_{i,\star}),$$ Meaning that any added noise s.t  $p_{ij}+e_j>p_{ij^*}+e_{j^*}$ where $y_{j^*}$ is the true corresponding point, yield a wrong solution, regardless to a proximity or relation between $y_j$ and $y_{j^*}$.

We notate $\softP$ as the soft correspondence mapping at the initial state, while $\softP^*$ is the refined soft alignment we wish to extract at the end of the denoising phase. We assume there is a noise matrix $E\in \mathbb{R}^{N\times M}$ of the graph signals such that
\begin{equation}
    \softP = \softP^* + E
\end{equation}

Without prior information on $\softP^*$, it is impossible to restore the underlying signals. Fortunately, the most known priors for the graph denoising problem fit our situation; those priors are feature space sparsity and node pair-wise smoothness.\\
We follow Chen \etal \cite{chen2020graph} notation of graph filters for graph denosing:
\begin{equation}\label{eq:graphobj}
    \softP^{*} = \mathbb{H} * \bm{s} = \sum_{l=1}^{L}(\mathbb{H}_lA^ls)
\end{equation}
Where $\bm{s}$ is the initial graph signal, $*$ is the graph convolution operator, and $\mathbb{H}_{l}$ are $L$ layers of Graph filter coefficients.
For stability reasons one might decide to use the residual objective as in our case:
\begin{equation}\label{eq:graphobj}
    \softP^{*} = \bm{s} + \mathbb{H} * \bm{s} = \bm{s} + \sum_{l=1}^{L}(\mathbb{H}_lA^ls)
\end{equation}
Meaning we try to infer $-E$ explicitly and subtract it from the initial noisy graph input.
In our work $\mathbb{H}$ will be the $GDC$ convolution layer \ref{subsec:GDC}, and $\bm{s}\coloneqq\softP$.\\
Solving \ref{eq:graphobj} requires formulating the objective as an optimization function. Using our priors on $\softP^{*}$ we have:
\begin{equation}\label{eq:graphlossv1}
\begin{aligned}
     \mathcal{L}_L = {\softP^{*}}^T&L\softP^{*} \quad
    \mathcal{L}_{l1} = ||\softP^{*}\mathbbm{1}||_1 \\
    \softP^{*} = \min_{\softP^{*}} ||&\softP^{i}-\softP^{*}||_2^2 + \alpha\mathcal{L}_L + \beta \mathcal{L}_{l1} \\
    s.t \quad &\softP^{*} = \softP + \mathbb{H} * \softP.
\end{aligned}
\end{equation}
The first term enforces $\softP^{*}$ not to diverge from the source signal, while terms 2,3 act as the graph denoisers. $L$ is the graph Laplacian matrix $L=D-A\in\mathbb{R}^{N\times N}$ with diagonal degree matrix $D_{i,i}=|N(i)|$ and $A$ as the adjacency matrix.






==> eso-pic.sty.tex <==
%%
%% This is file `eso-pic.sty',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% eso-pic.dtx  (with options: `package')
%% 
%% This is a generated file.
%% 
%% Copyright (C) 1998-2002 by Rolf Niepraschk <niepraschk@ptb.de>
%% 
%% This file may be distributed and/or modified under the conditions of
%% the LaTeX Project Public License, either version 1.2 of this license
%% or (at your option) any later version.  The latest version of this
%% license is in:
%% 
%%    http://www.latex-project.org/lppl.txt
%% 
%% and version 1.2 or later is part of all distributions of LaTeX version
%% 1999/12/01 or later.
%% 
\NeedsTeXFormat{LaTeX2e}[1999/12/01]
\ProvidesPackage{eso-pic}
   [2002/11/16 v1.1b eso-pic (RN)]
\input{iccv_eso.sty}
\newcommand\LenToUnit[1]{#1\@gobble}

\newcommand\AtPageUpperLeft[1]{%
  \begingroup
    \@tempdima=0pt\relax\@tempdimb=\ESO@yoffsetI\relax
    \put(\LenToUnit{\@tempdima},\LenToUnit{\@tempdimb}){#1}%
  \endgroup
}
\newcommand\AtPageLowerLeft[1]{\AtPageUpperLeft{%
  \put(0,\LenToUnit{-\paperheight}){#1}}}
\newcommand\AtPageCenter[1]{\AtPageUpperLeft{%
  \put(\LenToUnit{.5\paperwidth},\LenToUnit{-.5\paperheight}){#1}}%
}
\newcommand\AtTextUpperLeft[1]{%
  \begingroup
    \setlength\@tempdima{1in}%
    \ifodd\c@page%
      \advance\@tempdima\oddsidemargin%
    \else%
      \advance\@tempdima\evensidemargin%
    \fi%
    \@tempdimb=\ESO@yoffsetI\relax\advance\@tempdimb-1in\relax%
    \advance\@tempdimb-\topmargin%
    \advance\@tempdimb-\headheight\advance\@tempdimb-\headsep%
    \put(\LenToUnit{\@tempdima},\LenToUnit{\@tempdimb}){#1}%
  \endgroup
}
\newcommand\AtTextLowerLeft[1]{\AtTextUpperLeft{%
  \put(0,\LenToUnit{-\textheight}){#1}}}
\newcommand\AtTextCenter[1]{\AtTextUpperLeft{%
  \put(\LenToUnit{.5\textwidth},\LenToUnit{-.5\textheight}){#1}}}
\newcommand{\ESO@HookI}{} \newcommand{\ESO@HookII}{}
\newcommand{\ESO@HookIII}{}
\newcommand{\AddToShipoutPicture}{%
  \@ifstar{\g@addto@macro\ESO@HookII}{\g@addto@macro\ESO@HookI}}
\newcommand{\ClearShipoutPicture}{\global\let\ESO@HookI\@empty}
\newcommand\ESO@isMEMOIR[1]{}
\@ifclassloaded{memoir}{\renewcommand\ESO@isMEMOIR[1]{#1}}{}
\newcommand{\@ShipoutPicture}{%
  \bgroup
    \@tempswafalse%
    \ifx\ESO@HookI\@empty\else\@tempswatrue\fi%
    \ifx\ESO@HookII\@empty\else\@tempswatrue\fi%
    \ifx\ESO@HookIII\@empty\else\@tempswatrue\fi%
    \if@tempswa%
      \@tempdima=1in\@tempdimb=-\@tempdima%
      \advance\@tempdimb\ESO@yoffsetI%
      \ESO@isMEMOIR{%
        \advance\@tempdima\trimedge%
        \advance\@tempdima\paperwidth%
        \advance\@tempdima-\stockwidth%
        \if@twoside\ifodd\c@page\else%
          \advance\@tempdima-2\trimedge%
          \advance\@tempdima-\paperwidth%
          \advance\@tempdima\stockwidth%
        \fi\fi%
        \advance\@tempdimb\trimtop}%
      \unitlength=1pt%
      \global\setbox\@cclv\vbox{%
        \vbox{\let\protect\relax
          \pictur@(0,0)(\strip@pt\@tempdima,\strip@pt\@tempdimb)%
            \ESO@HookIII\ESO@HookI\ESO@HookII%
            \global\let\ESO@HookII\@empty%
          \endpicture}%
          \nointerlineskip%
        \box\@cclv}%
    \fi
  \egroup
}
\EveryShipout{\@ShipoutPicture}
\RequirePackage{keyval}
\newif\ifESO@dvips\ESO@dvipsfalse \newif\ifESO@grid\ESO@gridfalse
\newif\ifESO@texcoord\ESO@texcoordfalse
\newcommand*\ESO@gridunitname{}
\newcommand*\ESO@gridunit{}
\newcommand*\ESO@labelfactor{}
\newcommand*\ESO@griddelta{}\newcommand*\ESO@griddeltaY{}
\newcommand*\ESO@gridDelta{}\newcommand*\ESO@gridDeltaY{}
\newcommand*\ESO@gridcolor{}
\newcommand*\ESO@subgridcolor{}
\newcommand*\ESO@subgridstyle{dotted}% ???
\newcommand*\ESO@gap{}
\newcommand*\ESO@yoffsetI{}\newcommand*\ESO@yoffsetII{}
\newcommand*\ESO@gridlines{\thinlines}
\newcommand*\ESO@subgridlines{\thinlines}
\newcommand*\ESO@hline[1]{\ESO@subgridlines\line(1,0){#1}}
\newcommand*\ESO@vline[1]{\ESO@subgridlines\line(0,1){#1}}
\newcommand*\ESO@Hline[1]{\ESO@gridlines\line(1,0){#1}}
\newcommand*\ESO@Vline[1]{\ESO@gridlines\line(0,1){#1}}
\newcommand\ESO@fcolorbox[4][]{\fbox{#4}}
\newcommand\ESO@color[1]{}
\newcommand\ESO@colorbox[3][]{%
  \begingroup
    \fboxrule=0pt\fbox{#3}%
  \endgroup
}
\newcommand\gridSetup[6][]{%
  \edef\ESO@gridunitname{#1}\edef\ESO@gridunit{#2}
  \edef\ESO@labelfactor{#3}\edef\ESO@griddelta{#4}
  \edef\ESO@gridDelta{#5}\edef\ESO@gap{#6}}
\define@key{ESO}{texcoord}[true]{\csname ESO@texcoord#1\endcsname}
\define@key{ESO}{pscoord}[true]{\csname @tempswa#1\endcsname
  \if@tempswa\ESO@texcoordfalse\else\ESO@texcoordtrue\fi}
\define@key{ESO}{dvips}[true]{\csname ESO@dvips#1\endcsname}
\define@key{ESO}{grid}[true]{\csname ESO@grid#1\endcsname
  \setkeys{ESO}{gridcolor=black,subgridcolor=black}}
\define@key{ESO}{colorgrid}[true]{\csname ESO@grid#1\endcsname
  \setkeys{ESO}{gridcolor=red,subgridcolor=green}}
\define@key{ESO}{gridcolor}{\def\ESO@gridcolor{#1}}
\define@key{ESO}{subgridcolor}{\def\ESO@subgridcolor{#1}}
\define@key{ESO}{subgridstyle}{\def\ESO@subgridstyle{#1}}%
\define@key{ESO}{gridunit}{%
  \def\@tempa{#1}
  \def\@tempb{bp}
  \ifx\@tempa\@tempb
    \gridSetup[\@tempa]{1bp}{1}{10}{50}{2}
  \else
    \def\@tempb{pt}
    \ifx\@tempa\@tempb
      \gridSetup[\@tempa]{1pt}{1}{10}{50}{2}
    \else
      \def\@tempb{in}
      \ifx\@tempa\@tempb
        \gridSetup[\@tempa]{.1in}{.1}{2}{10}{.5}
      \else
        \gridSetup[mm]{1mm}{1}{5}{20}{1}
      \fi
    \fi
  \fi
}
\setkeys{ESO}{subgridstyle=solid,pscoord=true,gridunit=mm}
\def\ProcessOptionsWithKV#1{%
  \let\@tempc\@empty
  \@for\CurrentOption:=\@classoptionslist\do{%
    \@ifundefined{KV@#1@\CurrentOption}%
    {}{\edef\@tempc{\@tempc,\CurrentOption,}}}%
  \edef\@tempc{%
    \noexpand\setkeys{#1}{\@tempc\@ptionlist{\@currname.\@currext}}}%
  \@tempc
  \AtEndOfPackage{\let\@unprocessedoptions\relax}}%
\ProcessOptionsWithKV{ESO}%
\newcommand\ESO@div[2]{%
  \@tempdima=#1\relax\@tempdimb=\ESO@gridunit\relax
  \@tempdimb=#2\@tempdimb\divide\@tempdima by \@tempdimb%
  \@tempcnta\@tempdima\advance\@tempcnta\@ne}
\AtBeginDocument{%
  \IfFileExists{color.sty}
  {%
    \RequirePackage{color}
    \let\ESO@color=\color\let\ESO@colorbox=\colorbox
    \let\ESO@fcolorbox=\fcolorbox
  }{}
  \@ifundefined{Gin@driver}{}%
  {%
    \ifx\Gin@driver\@empty\else%
      \filename@parse{\Gin@driver}\def\reserved@a{dvips}%
      \ifx\filename@base\reserved@a\ESO@dvipstrue\fi%
    \fi
  }%
  \ifx\pdfoutput\undefined\else
    \ifx\pdfoutput\relax\else
      \ifcase\pdfoutput\else
        \ESO@dvipsfalse%
      \fi
    \fi
  \fi
  \ifESO@dvips\def\@tempb{eepic}\else\def\@tempb{epic}\fi
  \def\@tempa{dotted}%\def\ESO@gap{\LenToUnit{6\@wholewidth}}%
  \ifx\@tempa\ESO@subgridstyle
    \IfFileExists{\@tempb.sty}%
    {%
      \RequirePackage{\@tempb}
      \renewcommand*\ESO@hline[1]{\ESO@subgridlines\dottedline{\ESO@gap}%
        (0,0)(##1,0)}
      \renewcommand*\ESO@vline[1]{\ESO@subgridlines\dottedline{\ESO@gap}%
        (0,0)(0,##1)}
    }{}
  \else
    \ifx\ESO@gridcolor\ESO@subgridcolor%
      \renewcommand*\ESO@gridlines{\thicklines}
    \fi
  \fi
}
\ifESO@texcoord
  \def\ESO@yoffsetI{0pt}\def\ESO@yoffsetII{-\paperheight}
  \edef\ESO@griddeltaY{-\ESO@griddelta}\edef\ESO@gridDeltaY{-\ESO@gridDelta}
\else
  \def\ESO@yoffsetI{\paperheight}\def\ESO@yoffsetII{0pt}
  \edef\ESO@griddeltaY{\ESO@griddelta}\edef\ESO@gridDeltaY{\ESO@gridDelta}
\fi
\newcommand\ESO@gridpicture{%
  \begingroup
    \setlength\unitlength{\ESO@gridunit}%
    \ESO@color{\ESO@subgridcolor}%
    \ESO@div{\paperheight}{\ESO@griddelta}%
    \multiput(0,0)(0,\ESO@griddeltaY){\@tempcnta}%
      {\ESO@hline{\LenToUnit{\paperwidth}}}%
    \ESO@div{\paperwidth}{\ESO@griddelta}%
    \multiput(0,\LenToUnit{\ESO@yoffsetII})(\ESO@griddelta,0){\@tempcnta}%
      {\ESO@vline{\LenToUnit{\paperheight}}}%
    \ESO@color{\ESO@gridcolor}%
    \ESO@div{\paperheight}{\ESO@gridDelta}%
    \multiput(0,0)(0,\ESO@gridDeltaY){\@tempcnta}%
      {\ESO@Hline{\LenToUnit{\paperwidth}}}%
    \ESO@div{\paperwidth}{\ESO@gridDelta}%
    \multiput(0,\LenToUnit{\ESO@yoffsetII})(\ESO@gridDelta,0){\@tempcnta}%
      {\ESO@Vline{\LenToUnit{\paperheight}}}%
    \fontsize{10}{12}\normalfont%
    \ESO@div{\paperwidth}{\ESO@gridDelta}%
    \multiput(0,\ESO@gridDeltaY)(\ESO@gridDelta,0){\@tempcnta}{%
      \@tempcntb=\@tempcnta\advance\@tempcntb-\@multicnt%
      \ifnum\@tempcntb>1\relax
        \multiply\@tempcntb by \ESO@gridDelta\relax%
        \@tempdima=\@tempcntb sp\@tempdima=\ESO@labelfactor\@tempdima%
        \@tempcntb=\@tempdima%
        \makebox(0,0)[c]{\ESO@colorbox{white}{\the\@tempcntb}}%
      \fi}%
    \ifx\ESO@gridunitname\@empty\def\@tempa{0}\else\def\@tempa{1}\fi%
    \ESO@div{\paperheight}{\ESO@gridDelta}%
    \multiput(\ESO@gridDelta,0)(0,\ESO@gridDeltaY){\@tempcnta}{%
      \@tempcntb=\@tempcnta\advance\@tempcntb-\@multicnt%
      \ifnum\@tempcntb>\@tempa\relax
        \multiply\@tempcntb by \ESO@gridDelta\relax%
        \@tempdima=\@tempcntb sp\@tempdima=\ESO@labelfactor\@tempdima%
        \@tempcntb=\@tempdima%
        \makebox(0,0)[c]{\ESO@colorbox{white}{\the\@tempcntb}}%
      \fi
    }%
    \ifx\ESO@gridunitname\@empty\else%
      \thicklines\fboxrule=\@wholewidth%
      \put(\ESO@gridDelta,\ESO@gridDeltaY){\makebox(0,0)[c]{%
        \ESO@fcolorbox{\ESO@gridcolor}{white}{%
          \textbf{\ESO@gridunitname}}}}%
    \fi
    \normalcolor%
  \endgroup
}
\ifESO@grid\g@addto@macro\ESO@HookIII{\ESO@gridpicture}\fi
\endinput
%%
%% End of file `eso-pic.sty'.


==> title_up.tex <==
% \begin{strip}


% \centering\noindent

% \vspace{-50pt}
% \begin{subfigure}{0.19\textwidth}
% \captionsetup{justification=centering}
%   \includegraphics[width=\linewidth]{Sections/Abstract/tizer_pairs/faust_teezer.png}
%   \captionof*{figure}{Non-isometric}

%   \label{fig:1}
% \end{subfigure}\hfil % <-- added
% \begin{subfigure}{0.30\textwidth}
% \vspace{40pt}
%   \includegraphics[width=\linewidth]{Sections/Abstract/tizer_pairs/animals.png}
%   \captionof*{figure}{Multi-class}
%   \label{fig:2}
% \end{subfigure}\hfil % <-- added
% \begin{subfigure}{0.28\textwidth}
% \vspace{20pt}
%   \includegraphics[width=\linewidth]{Sections/Abstract/tizer_pairs/point_cloud.png}
%   \captionof*{figure}{Various topologies}
%   \label{fig:1}
% \end{subfigure}\hfil 
% \label{fig:tizerpairs}%
% \captionsetup{justification=centering}
% \captionof{figure}{We present DG2N - a self-supervised zero-shot iterative mechanism for dense shape correspondence. Built on top of a naive all-to-all mapping, we construct a deep network that uses the inverse projection probability between graphs as features in a learnable iterative scheme. This novel design is a template-free, unsupervised, learnable algorithm which is capable of aligning meshes and point clouds under non-rigid deformation, such as isometric, stretchable or even different classes and different topologies. We report here state-of-the-art results on multiple data-sets, as well as outlier-free alignments.}


% \end{strip}

\twocolumn[{%
\renewcommand\twocolumn[1][]{#1}%
\maketitle
\begin{center}
    \centering
    \includegraphics[width=.9\textwidth,height=5cm]{tizzer_figure.png}
    \captionof{figure}{We present DG2N - a self-supervised zero-shot iterative mechanism for dense shape correspondence. Built on top of an initial all-to-all mapping, we construct a deep network that uses the projected probabilities between graphs as features in a learnable iterative scheme. This novel design is a template-free, unsupervised, learnable algorithm which is capable of aligning meshes and point clouds under non-rigid deformation, such as isometric, stretchable or even different classes and different topologies. We report here state-of-the-art results on multiple data-sets, as well as outlier-free alignments.}
\end{center}%
}]

